SQUASH: Simple QoS-Aware High-Performance Memory Scheduler for Heterogeneous Systems with Hardware Accelerators

Modern SoCs integrate multiple CPU cores and Hardware Accelerators (HWAs) that share the same main memory system, causing interference among memory requests from different agents. The result of this interference, if not controlled well, is missed deadlines for HWAs and low CPU performance. State-of-the-art mechanisms designed for CPU-GPU systems strive to meet a target frame rate for GPUs by prioritizing the GPU close to the time when it has to complete a frame. We observe two major problems when such an approach is adapted to a heterogeneous CPU-HWA system. First, HWAs miss deadlines because they are prioritized only close to their deadlines. Second, such an approach does not consider the diverse memory access characteristics of different applications running on CPUs and HWAs, leading to low performance for latency-sensitive CPU applications and deadline misses for some HWAs, including GPUs. In this paper, we propose a Simple Quality of service Aware memory Scheduler for Heterogeneous systems (SQUASH), that overcomes these problems using three key ideas, with the goal of meeting deadlines of HWAs while providing high CPU performance. First, SQUASH prioritizes a HWA when it is not on track to meet its deadline any time during a deadline period. Second, SQUASH prioritizes HWAs over memory-intensive CPU applications based on the observation that the performance of memory-intensive applications is not sensitive to memory latency. Third, SQUASH treats short-deadline HWAs differently as they are more likely to miss their deadlines and schedules their requests based on worst-case memory access time estimates. Extensive evaluations across a wide variety of different workloads and systems show that SQUASH achieves significantly better CPU performance than the best previous scheduler while always meeting the deadlines for all HWAs, including GPUs, thereby largely improving frame rates.

==> sections/background-lavanya.tex <==

\section{Background}

In this section, we will first provide a brief background on the
organization of the DRAM main memory system and memory scheduling
techniques employed in CPU-only multicore systems. We will then
describe the memory access characteristics of hardware
accelerators (HWAs) and the closest previous works on managing
memory bandwidth in heterogeneous systems that integrate CPUs and
hardware accelerators (HWAs).

\subsection{DRAM Organization}

% I modified this section to be top-down, starting with channels.
% Also, I made the description more high level because I think
% that suits a memory scheduling paper better. We can discuss if
% you have concerns or questions.

A modern DRAM memory system is organized as channels, ranks and
banks in a hierarchical manner. Each channel has its own address
and data bus and operates independently. A channel consists of one
or more ranks. A rank, in turn, consists of multiple banks. Each
bank can operate independently in parallel with the other banks.
However, all the banks on a channel share the address and data bus
of the channel.

Each bank is organized as a two dimensional array of rows and
columns. When a piece of data is accessed from a bank, the entire
row (~4KB) containing the piece of data is brought into an
internal structure called the row buffer. A subsequent access to
data in the same row can be served from the row buffer itself and
need not access the array. Such an access is called a \emph{row
hit}. On the other hand, if the subsequent access is to data in a
different row, the array needs to be accessed and the new row
needs to be brought into the row buffer. Such an access is called
a \emph{row miss}. A \emph{row miss} incurs more than 2x the
latency of a row hit.


\subsection{DRAM Scheduling in CPU-only systems}

Previous work has proposed to take advantage of the row
buffer and row hit behavior. The First-Ready
First-Come-First-Served (FRFCFS)~\cite{frfcfs} scheduler prioritizes row hits
over row misses and older requests, to ensure forward progress.
While such a scheme maximizes DRAM bandwidth utilization, it
unfairly prioritizes applications with high row-buffer locality
(large number of requests to the same row) and high
memory-intensity (large number of requests to main memory),
causing interference to other applications. 

Previous work~\cite{parbs,atlas,tcm} has proposed application-aware memory
request scheduling to mitigate interference between applications
at the main memory. The basic idea behind application-aware memory
scheduling is to take into account applications' memory access
characteristics and reorder requests at the memory controller such
that inter-application interference is mitigated and performance
is improved. A recent previous work, Thread Cluster Memory scheduling
(TCM), proposed to separate applications into non-intensive and
intensive clusters based on their memory access intensity and
prioritize requests from the non-intensive cluster over requests
from the intensive cluster. 

% I am not sure if the paragraph below needs to be in background. We could
% move it to the related work section.

%Other previous works have proposed techniques to guarantee a
%minimum bandwidth requirement and a maximum response time bound
%for the main memory. A Predictable SDRAM Memory Controller
%(Predator)~\cite{predator} proposes to group a series of read or
%write requests that access a bank and schedule each group of
%requests together. Credit-Controlled Static Priority (CCSP)
%arbiter~\cite{ccsp} proposes to schedule requests at the memory
%controller using a rate-based regulation scheme and a static
%priority scheduler, with the goal of guaranteeing a minimum
%bandwidth requirement and a maximum response time limit for each
%requestor. Yun proposed Memguard~\cite{memguard} that divided
%memory bandwidth into two components - a guaranteed component and
%a best-effort component. A certain guaranteed component of
%bandwidth is ensured for each core. After each core consumes its
%guaranteed bandwidth, the remaining bandwidth is used to achieve
%good performance, in a best-effort manner.

\subsection{Hardware Accelerator Characteristics}

HWAs are designed for accelerating specific functions and have
very different memory access patterns than CPU cores. There are a
wide variety of HWAs integrated onto current SoCs. The functions
that they accelerate are diverse and the implementations are also
very various. We will describe a 3x3 horizontal Sobel filter
accelerator and its characteristics as an example.

\begin{figure}
  \centering
  \includegraphics[scale=0.35, angle=0]{figs/fig_hwa}
  \caption{Typical Implementation of Sobel Filter HWA}
  \label{fig:HWAexample}
\end{figure}

The accelerator executes the Sobel filter on a target VGA
(640x480) image, at a frame rate of 30 frames per second (fps). A
typical implementation for a 3x3 filter uses line memories to
take advantage of data access locality and hide the memory access latency,
as shown in Figure~\ref{fig:HWAexample}. The line memory
(consisting of lines A, B, C and D) can hold four lines, each of
size 640 pixels, of the target image. The filter operates on three
lines, at any point in time, while the next line is being
prefetched. For instance, the filter operates on lines A, B and C,
while line D is being prefetched. After the filter finishes
processing lines A, B and C, it operates on lines B, C and D,
while line A is being prefetched. As long as the next line is
prefetched while the filter is operating on the three previous
rows, memory access latency does not affect performance. To meet
a target performance, say, 30 frames per second (fps), the
filtering operation on a set of lines and fetching the next line
have to be finished within 69.44 usec. In this case, the period of
the HWA is 69.44 usec and requests generated to pre(fetch) the
next line need to be completed by the 69.44 usec deadline. A
deadline miss causes the filtering logic to stall and prevents the
system from achieving the target performance.

On the other hand, if the (pre)fetch of the next line is finished
earlier than the deadline, the prefetch of the line after that
cannot be initiated, since the line memory can only hold one extra
prefetched line. Prefetching more than one line can overwrite the
contents of the line that is currently being processed by the
filter logic. In order to provision for more capacity to hold
prefetched data and hide memory latency better, double buffers, like the
frame buffers, used in computer graphics, are also used in some
HWAs. The amount of available buffer capacity determines the
deadline/period of the HWA. However, in all these cases, the HWA
requires a certain amount of consistent bandwidth, in order to
meet the target performance. For instance, in the example
described above, the HWA requires consistent bandwidth during each
period (640 bytes for every 69.44 usec). As long as this
consistent bandwidth is allocated, the HWA is tolerant of memory
latency. Furthermore, finishing the HWA's memory accesses earlier
than the deadline is wasteful, especially in a system with other
agents such as CPU cores, where the memory bandwidth can be better
utilized to achieve higher overall performance for the other
agents. In fact, a major challenge in today's heterogeneous
SoC-like systems is to ensure that HWAs get a consistent share of
memory bandwidth such that their deadlines are met, while still
allocating enough bandwidth to the CPU cores, to achieve high
overall system performance.

\subsection{DRAM scheduling in Heterogeneous System}

One previous work~\cite{armwhite} attempts to tackle this problem
by acknowledging the differences in memory access characteristics
of different agents in an SoC. CPU cores are latency sensitive,
while the GPU and Video Processing Unit (VPU) that accelerates
video decoding and encoding, are bandwidth sensitive and have
better memory latency tolerance. Therefore, as long as sufficient bandwidth
is consistently provided to the GPU and VPU over a period of time,
they can meet their target performance. Based on these
characteristics, they proposed techniques to regulate the amount
of outstanding GPU bandwidth demand and prioritize CPU requests
over GPU requests. However, if CPU applications require large
bandwidth, the GPU's target performance is often not 
satisfied~\cite{schedulingCPUGPU}. In contrast, always
prioritizing the GPU over CPU cores can enable the GPU to meet its
target frame rate. However, such a scheme would cause significant
interference to the CPU cores.

In order to address this challenge, previous
work~\cite{schedulingCPUGPU} has proposed to dynamically adjust
memory access priorities between the CPU cores and the GPU. This
policy compares the current progress in terms of tiles rendered in
a frame (Equation~\ref{eq:FrameProgress}) against expected
progress in terms of time elapsed in a period
(Equation~\ref{eq:ExpectedProgress} and adjusts priorities.

\begin{equation}
CurrentProgress = \frac{Number\ of\ tiles\ rendered}{Number\ of\ tiles\ in the frame} 
\label{eq:FrameProgress}
\end{equation}
\begin{equation}
ExpectedProgress = \frac{Time\ elapsed\ in\ the\ current\ frame}{Period\ for\ each\ frame}
\label{eq:ExpectedProgress}
\end{equation}

When {\it CurrentProgress} is greater than {\it ExpectedProgress},
the GPU is on track to meet the target frame rate. Hence, the GPU
is given lower priority than the CPU. On the other hand, if the
{\it CurrentProgress} is less than {\it ExpectedProgress}, the GPU
is not on track to meet the target frame rate. In order to enable
the GPU to make better progress, it's requests are given the same
priority as the CPU cores' requests. Only when the {\it
ExpectedProgress} is greater than an {\it EmergentThreshold}
(=0.90), are the GPU's requests given higher priority than the CPU
cores' requests. Such a policy guarantees a consistent average
bandwidth to the GPU and reduces the number of times it misses a
deadline, while providing high CPU performance.










==> sections/deadline_results_gpu.tex <==
\begin{table}[ht]
\scriptsize
\centering
\setlength{\tabcolsep}{.60em}
    \begin{tabular}{lcc}
      \toprule
      \multirow{2}{*}{\textbf{\begin{minipage}{0.5in}Scheduling Algorithms\end{minipage}}} &
      \textbf{Deadline-Met Ratio (\%) / Frame Rate (fps)} \\
       & MAT \\
      \midrule
      FRFCFS-DynOpt & 99.999 / 29.83 \\
%      SQ-NoProb & 100 / 30 & 100 / 30 \\
      SQUASH & 100 / 30 \\
      \bottomrule
    \end{tabular}
\vspace{-1mm}
\caption{Deadline-met ratio and frame rate of HWAs}
\label{tab:gpu_hwa_performance}%
\end{table}


==> sections/evaluation-bak.tex <==
\section{Evaluation}\label{sec:evaluation} We compare SQUASH
with previously proposed schedulers, FRFCFS and TCM with static priority
(FRFCFS-St, TCM-St), FRFCFS with \emph{Dyn-Prio} (FRFCFS-Dyn). Static priority
always sets higher priority to all HWAs than all CPUs. We use {\it
EmergentThreshold} of 0.9 and 0.3 for FRFCFS-Dyn.

%Schedulers with dynamic priority adjusts priority dynamically based on the
%progress of the HWA \cite{schedulingCPUGPU}. In order to anaylyze benefits of
%SQUASH, we evaluate schedulings that employ only \emph{Dist-Prio} to FRFCFS
%(SQUASH-FDist) and TCM (SQUASH-TDist). FRFCFS with dynamic distributed
%priority, (FRFCFS-DynD) TCM with static priority (TCM-St), TCM with dynamic
%distributed priority (TCM-DynD). When {\it CurrentProgress} is greater than
%{\it ExpectedProgress}, FRFCFS-Dyn sets the priority of a HWA to the same as
%CPUs, but FRFCFS-DynD and TCM-DynD set the priority of HWA higher than CPUs.

\subsection{Multicore Results} Figure \ref{plot:average_performance} shows the
averaged system performance and fairness of six schedulers across all 80
workloads using Config-A and B. Table \ref{tab:average_hwa_performance} shows
deadline-met ratio and frame rate of four types of HWAs (IMG-HWAs satisfy target
performance with all schedulers). We assume that any deadline misses of a frame
drop the frame in order to calculate the frame rates.

\begin{figure}[ht!]
  \flushleft
  \begin{minipage}{0.23\textwidth}
    \flushleft
    \includegraphics[scale=0.17, angle=270]{plots/main_avg_unnorm_ws}
  \end{minipage}
%  \begin{minipage}{0.32\textwidth}
%    \flushleft
%    \includegraphics[scale=0.22, angle=270]{plots/main_avg_unnorm_hs}
%  \end{minipage}
  \begin{minipage}{0.23\textwidth}
    \flushleft
    \includegraphics[scale=0.17, angle=270]{plots/main_avg_unnorm_ms}
  \end{minipage}
  \caption{System performance and fairness of SQUASH and proposed schedulers}
  \label{plot:average_performance}
\end{figure}

\input{sections/deadline_results}

%\begin{table}[h!]
%\begin{scriptsize}
%\begin{tiny}
%  \centering
%  \begin{tabular}{|l|l|l|l|l|l|l|l|l|}
%    \hline
%    Scheduling & \multicolumn{4}{l}{Met Rate (\%)} & \multicolumn{4}{|l|}{frame rate (fps)} \\
%    \cline{2-9}
%    & HES & MAT & RSZ & DET & HES & MAT & RSZ & DET \\
%    \hline
%    FRFCFS-St & 100 & 100 & 100 & 100 & 30 & 30 & 30 & 30 \\
%    \hline
%    FRFCFS-Dyn0.9 & 99.52 & 53.16 & 99.62 & 98.77 & 16.31 & 16.22 & 28.88 & 23.25 \\
%    \hline
%    FRFCFS-Dyn0.3 & 99.996 & 97.13 & 100 & 100 & 27.84 & 26.25 & 30 & 30 \\
%    \hline
%    SQUASH-FDist & 99.91 & 99.999 & 100 & 99.72 & 17.81 & 29.81 & 30 & 23.06 \\
%    \hline
%    TCM-St & 100 & 100 & 100 & 100 & 30 & 30 & 30 & 30 \\
%    \hline
%    SQUASH-TDist & 99.94 & 100 & 100 & 99.74 & 16.97 & 29.91 & 30 & 23.06 \\
%    \hline
%    SQUASH & 100 & 100 & 100 & 100 & 30 & 30 & 30 & 30\\
%    \hline
%    SQUASH-Prob & 100 & 100 & 100 & 100 & 30 & 30 & 30 & 30\\
%    \hline
%  \end{tabular}
%  \caption{Deadline met ratio and frame rate of HWAs with SQUASH and proposed schedulers}
%  \label{tab:average_hwa_performance}
%  \end{scriptsize}
%  \end{tiny}
%\end{table}

%\begin{figure}[ht!]
%  \centering
%  \begin{minipage}{0.23\textwidth}
%    \centering
%    \includegraphics[scale=0.17, angle=270]{plots/main_avg_metratio}
%  \end{minipage}
%  \begin{minipage}{0.23\textwidth}
%    \centering
%    \includegraphics[scale=0.17, angle=270]{plots/main_avg_fps}
%  \end{minipage}
%  \caption{Deadline met ratio and frame rate of HWAs with SQUASH and proposed schedulers}
%  \label{plot:average_hwa_performance}
%\end{figure}

We make two observations.
%First, FRFCFS-St and TCM-St also can keep dealines for HWAs, but they shows
%much worse performance than the other schedulings that adjust priorities
%dynamically. This is because HWAs always interfere the all CPUs with static
%priority scheduling and performance of memory non-intensive application is
%degraded much. It shows that adjusting priorities dynamically is needed in
%CPU-HWA systems.
First, SQUASH achieves 15.5\% better weighted speedup than FRFCFS-Dyn0.3 while
keeping the deadline met ratio 100\%. FRFCFS-Dyn0.9 shows almost the same
performance as SQUASH, but deadline-met ratio of MAT-HWA is quite low (only
53.16\%). The same priority between HWAs and CPUs is insufficient to give enough
bandwidth to HWAs. Smaller {\it EmergentThreshold} causes long consecutive
cycles that HWAs have high priority and they delay CPUs significantly.

Second, SQUASH-Prob provide 22.5\% fairness improvement and only 0.5\% performance degradation over SQUASH due to preventing HWAs from over-prioritizing.
Fairness of SQUASH-Prob is 17.5\% worse than FRFCFS-Dyn0.3. Although system performance and fairness are trade-off each other, SQUASH-Prob improves system performance
while mitigating fairness degradation.

Next, we will breakdown the benefit of SQUASH into each factor.

%First, \emph{Dist-Prio} achives both high system performance and high deadline met ratio compared \emph{Dyn-Prio}.
%The ratio for MAT-HWA with FRFCFS-Dyn is only 97.13 \% with {\it EmergentThreshold} of 0.3, and the weighted speedup of SQUASH-FDist is 9.3\% greater than that of FRFCFS-Dyn0.3.
%FRFCFS-Dyn0.9 shows better performance than SQUASH-FDist, but deadline met ratio of MAT-HWA is quite low. \emph{Dyn-Prio} does not provide enough bandwidth to HWAs.
%
%Second, the performance improvement for SQUASH and SQUASH-Prob against SQUASH-TDist is about 1\%. This is becasue, when there is not much contension on the memory,
%HWAs can utilize a large amount of bandwidth even when it is deemed as non-urgend. Therefore, the benefit of application-aware dynamic priority is limited. The difference of performance between
%various memory intensities is described in detail in Section\ref{sec:intensity}.
%
%First, FRFCFS-Dyn shows good performance but deadline met ratio for MAT-HWA is quite lower than other schedulings. MAT-HWA demands large bandwidth, but FRFCFS-Dyn does not provide enough
%bandwidth to MAT-HWA because the priority for MAT-HWA is the same or lower than CPUs for 90\% of the period. In order to improve deadline met ratio, we have a choice to decrease {\it EmergentThreshold}
%for FRFCFS-Dyn. We evaluate it in Section~\ref{sec:emergentThrehsold}.
%
%Next, SQUASH-FDist and SQUASH-TDist improves deadline met ratio against FRFCFS-Dyn. Distributing high priority over period provide enough bandwidth to HWAs. on the other hand, system performance
%of SQUASH-FDist is 6.5\% lower than FRFCFS-Dyn, because HWA with high priority interfere CPUs. Performance of SQUASH-TDist is better than SQUASH-FDist due to awareness of memory characteristics for CPU applications, but still lower than FRFCFS-Dyn.
%
%Then, SQUASH and SQUASH-Prob achieves 4\% better weighted speedup than SQUASH-TDist while keeping 100\% deadline met ratio of HWAs, and the performance of SQUASH is also 1.5\% better than
%FRFCFS-Dyn. This performance improvement is attributed to reducing the amount of time that HWAs are judged urgent. Moreover, scheduling HES-HWA based on the worst case latency
%improve deadlien met ratio HES-HWA. Not only HES-HWA having short deadline but also MAT-HWA having long deadline keeps the deadline with SQUASH.
%This is because MAT-HWA can utilize more bandwidth with SQUASH than with SQUASH-TDist when it is not judged urgent.
%
%Third, SQUASH-TDist does not achieve 100\% deadline met ratio, but SQUASH and SQUASH-Prob achieves it. Scheduling based on worst-case memory latency succeeds in
%improving deadline met ratio. SQUASH-TDist sometimes fail the deadline because of bandwidth fluctuation.
%
%Finally, SQUASH degrades harmonic speedup by 11\% and fairness by 46\% than SQUASH-TDist. This is because long deadline HWAs always delay
%memory intensive applications with SQUASH. On the other hand, SQUASH-Prob improves
%harmonic speedup and fairness against SQUASH; 2.7\% worse Hamonic speedup and 13\% worse fairness than SQUASH-TDist.
%With SQUASH-Prob, switching priorities based on the HWA's progress is able to control bandwidth
%utilized by HWAs and memory intensive applications are sometimes prior to non-urgent HWAs. SQUASH-Prob achieves fairness improvement while keeping system performance.

%\subsection{Effect of Distributing High Priority}\label{sec:emergentThrehsold}.
%
%Figure~\ref{plot:emergent} shows weighted speedup and the deadline met ratio for MAT-HWA for different values of {\it EmergentThreshold} across 25 workloads.
%Larger theshold value improves the deadline met ratio for FRFCFS-Dyn, but when threshold is even 0.3, deadline met ratio is only 93.5\%. Moreover, larger threshold value
%degrade system performance heavily. When threshold is 0.3, weighted speedup of FRFCFS-Dyn is only 3.86 that is 84.2\% of SQUASH with 0.7 of threshold that shows 100\% deadline.
%Consequently, SQUASH achieve higher perormance while keeping deadline met ratio than FRFCFS-Dyn.

%\begin{figure}[ht!]
%  \centering
%  \begin{minipage}{0.23\textwidth}
%    \centering
%    \includegraphics[scale=0.17, angle=270]{plots/emth_ws}
%  \end{minipage}
%  \begin{minipage}{0.23\textwidth}
%    \centering
%    \includegraphics[scale=0.17, angle=270]{plots/emth_metmat}
%  \end{minipage}
%  \caption{System performance and deadline met ratio for different {\it EmergentThreshold}}
%  \label{plot:emergent}
%\end{figure}

\subsection{Performance Breakdown of SQUASH} \label{sec:intensity}
Figure \ref{plot:intensity_results} shows system performance and fairness for different workload memory intensities
categorized based on the ratio of memory intensive workloads. In order to breakdown the benefit of SQUASH, we compare
additional three schedulers which are FRFCFS with \emph{Dist-Prio} (FRFCFS-Dist), TCM with \emph{Dist-Prio} (TCM-Dist),
TCM with \emph{Dist-Prio} and application-aware dynamic priorities for long-deadline HWA (TCM-DA). We do not evaluate
TCM with \emph{Dyn-Prio} because TCM ranks all CPUs strictly and it is hard to set HWAs the same priority as CPUs.
The performance and fairness are normalized with those of FRFCFS-Dyn0.3. The numbers above the bars of FRFCFS-Dyn0.3 show
 absolute values for FRFCFS-Dyn0.3.
Table \ref{tab:average_hwa_performance2} shows averaged deadline met ratio and frame rate of four types of HWAs that includes FRFCFS-Dist,
TCM-Dist and TCM-DA. We have five major conclusions for these results.

First, SQUASH and SQUASH-Prob achieve performance improvement for every intensity. Second, as memory intensity becomes more,
the system performance improvement of \emph{Dist-Prio} becomes greater (24\% at maximum). This is because, as the memory intensity of CPU workloads increases,
the bandwidth utilized by HWAs before {\it EmergentThreashold} decreases, due to the same priority of HWAs as CPUs. As result, after {\it EmergentThreshold}, HWAs consume
large amount of bandwidth and interfere CPU applications for a long time. On the other hand, \emph{Dist-Prio} provides high priotiy to HWAs with fine granularity and
HWAs interferes CPUs for shorter time than \emph{Dyn-Prio}.

Third, as memory intensity increases, the system performance improvement of TCM-DA against TCM-Dist becomes greater (8.2\% at maximum).
When memory intensity is high, CPU applications delay non-urgent HWA with \emph{Dist-Prio}.
As result, high priority ratio of HWA is increased and all CPUs are interfered by HWAs for a long time. Application-aware dynamic priority schcme
improves sytem performance by reducing high prioity ratio of HWAs.

Next, SQUASH shows as the almost same system performance as that of TCM-DA while keeping deadline met ratio of HES-HWA 100\%. Scheduling based on
the worst case latency improve deadline met ratio of short deadline HWAs with keeping high system performance.

Finally, SQUASH-Prob improves fairness for every intensity against SQUASH instead of a little performance degradation.
Therefore, We conclude that SQUASH-Prob provides better performance than the state-of-the-art memory scheduers while keeping deadline and applicaiton-aware
dynamic priority scheme improves system performance in high contention situation.

%Third, as memory intensity increases, fairness of SQUASH-Prob gets
%worse. The memory intensive applications
%are interfered by HWAs for a large amount of time and the lowest ranked CPU in the memory intensive applications can utilize too limited bandwidth, because the other higher
%ranked applications exahust the most of ramaining bandwidth. Consequently, the lowest ranked application is much delayed.
%However, when all applications are memory-intensive,
%SQUASH-Prob shows better fainess than TCM-St.

\begin{figure}[!t]
  \centering
  \begin{minipage}{0.23\textwidth}
    \centering
    \includegraphics[scale=0.17, angle=270]{plots/intensity_results_ws}
  \end{minipage}
%  \begin{minipage}{0.32\textwidth}
%    \centering
%    \includegraphics[scale=0.22, angle=270]{plots/intensity_results_hs}
%  \end{minipage}
  \begin{minipage}{0.23\textwidth}
    \centering
    \includegraphics[scale=0.17, angle=270]{plots/intensity_results_ms}
  \end{minipage}
  \caption{System performance and fairness of SQUASH for different workload memory intensities}
  \label{plot:intensity_results}
\end{figure}

\input{sections/deadline_results2}

%\subsection{Analysis HWA's execution with SQUASH}
%
In order to demonstrate the effect of SQUASH deeply, we show bandwidth utilized by HWA and priority ratio of the HWA in Figure \ref{plot:bw_ratio_hwa}.
The left grafh in Figure \ref{plot:bw_ratio_hwa} shows bandwidth utilized by memory non-intensive CPU applications, memory intensive CPU applications
and MAT-HWA when MAT-HWA is deemed as non-urgent. The right graph in Figure \ref{plot:bw_ratio_hwa} indicates priority ratio of the MAT-HWA.
These are averaged result over 80 workloads for config-A.
MAT-HWA demands 8.32 GB/s, but utilizes only 4.75 GB/s with TCM-Dist. Due to this over-deprioritizaton, MAT-HWA has high priority for 56\% of the execution time.
On the other hand, MAT-HWA utilizes 8.57 GB/s with SQUASH and it has high priority for only 14\% of the execution time. This reduction of the high priority improves
system performance on SQUASH. With SQUASH-Prob, memory-intensive applications utilize more bandwidth (3.0 GB/s) than that of SQUASH (2.1 GB/s).
In contrast, the bandwidth of MAT-HWA with SQUASH-Prob is 7.5 GB/s which is lower than the demands and the high priority ratio is increased to 29\%.
SQUASH-Prob decreases idle time than SQUASH (from 11\% to 6\%) due to preventing MAT-HWA from over-prioritizing. Consequently SQUASH-Prob shows
 slightly lower weighted speedup and much better fairness than those of SQUASH.

\begin{figure}[ht!]
  \centering
  \begin{minipage}{0.23\textwidth}
    \centering
    \includegraphics[scale=0.17, angle=270]{plots/main_avg_bw}
  \end{minipage}
  \begin{minipage}{0.23\textwidth}
    \centering
    \includegraphics[scale=0.17, angle=270]{plots/main_avg_ratio}
  \end{minipage}
  \caption{Bandwidth and Priority Ratio}
  \label{plot:bw_ratio_hwa}
\end{figure}


\subsection{Effect of HWAs' memory intensity}

We evaluate SQUASH and previously proposed schedulers for different HWAs' memory intensity. In this evaluation, 4 HWAs consists of 2 MAT-HWAs and 2 HES-HWAs
and we choose them from three configurations for each HWA.
With these HWAs, we execute two groups of workloads for CPU whose percentages of memory intensive workloads are 50 \% and 100 \%.
Table~\ref{tab:hwa_comb_config} shows detailed configurations. Each configuration has 6 combinations of HES-HWA.
We execute 5 CPU workloads for each combination.

\begin{table}[h!]
%\begin{scriptsize}
\begin{tiny}
  \centering
  \begin{tabular}{|l|l|l|l|l|l|}
    \hline
    Config. & CPU memory & M & M & N \\
    & intensity(\%) & (MAT-HWA1) & (MAT-HWA2) & (HES-HWAs) \\
    \hline
    50+L & 50 & 10 & 10 & 32,32 \\
    \cline{1-4}
    50+M & 50 & 10 & 20 & 32,64 \\
    \cline{1-4}
    50+H1 & 50 & 10 & 30 & 32,128 \\
    \cline{1-4}
    50+H2 & 50 & 20 & 20 & 64,64 \\
    \cline{1-4}
    100+L & 100 & 10 & 10 & 64,128 \\
    \cline{1-4}
    100+M & 100 & 10 & 20 & 128,128 \\
    \cline{1-4}
    100+H1 & 100 & 10 & 30 & \\
    \cline{1-4}
    100+H2 & 100 & 20 & 20 & \\
    \hline
    \end{tabular}
  \caption{Configuration of CPUs and HWAs}
  \label{tab:hwa_comb_config}
  \end{tiny}
%  \end{scriptsize}
\end{table}

Figure~\ref{plot:hwacomb_results} shows system performance and fairness normalized with FRFCFS-Dyn0.3. The numbers above the bars of FRFCFS-Dyn0.3 show
 absolute value for FRFCFS-Dyn0.3. We have three observations.
First, the more memory bandwidth HWAs need, the sytem performance improvement of SQUASH and SQUASH-Prob become greater (39\% at maximum).
This is because more memory intensive HWA is frequently deemed as urgent and delays the all CPUs. SQUASH can prevent from delaying
memory non-intensive applications and improve the performance. Second, SQUASH-Prob improve fairness against SQUASH across all workloads.
Third, the un-fairness of SQUASH and SQUASH-Prob get worse as memory intensity of HWAs increase because
memory intensive HWAs interfere memory intensive applications significantly.

%Third, at the configuration of 100+H2, only SQUASH-Prob improves system performance
%against SQUASH and TCM-DynD. In this case, memory non-intensive applications spend most of bandwidth and non-urgent HWAs cannot consume enough bandwidth even with SQUASH.
%Therefore, high priority cycles of HWA are still large with SQUASH. In contrast, SQUASH-Prob limits the bandwidth for memory non-intensive application and
%HWAs can utilize enough bandwidth. Consequently, high priority cycles of HWA is reduced and system performance is improved.

\begin{figure}[ht!]
  \centering
  \begin{minipage}{0.23\textwidth}
    \centering
    \includegraphics[scale=0.17, angle=270]{plots/hwa_config_results_ws}
  \end{minipage}
%  \begin{minipage}{0.32\textwidth}
%    \centering
%    \includegraphics[scale=0.22, angle=270]{plots/hwa_config_results_hs}
%  \end{minipage}
  \begin{minipage}{0.23\textwidth}
    \centering
    \includegraphics[scale=0.17, angle=270]{plots/hwa_config_results_ms}
  \end{minipage}
  \caption{System performance and fairness of SQUASH for different HWA configurations}
  \label{plot:hwacomb_results}
\end{figure}

Figure~\ref{plot:hwacomb_metratio} shows the deadline met ratio for HES-HWAs and MAT-HWAs. Over the all cases,
SQUASH and SQUASH-Prob keep the ratio of the HES-HWAs 100\%. For MAT-HWAs, SQUASH and SQUASH-Prob improves
the ratio over FRFCFS-Dyn0.3 by giving high priority at fine granularity.

\begin{figure}[ht!]
  \centering
  \begin{minipage}{0.23\textwidth}
    \centering
    \includegraphics[scale=0.17, angle=270]{plots/hwa_config_results_metratio}
  \end{minipage}
  \begin{minipage}{0.23\textwidth}
    \centering
    \includegraphics[scale=0.17, angle=270]{plots/hwa_config_results_metratio_mat}
  \end{minipage}
  \caption{Deadline met ratio HWAs with SQUASH for different HWA configurations}
  \label{plot:hwacomb_metratio}
\end{figure}

%\subsection{Effect of scheduling based on the worst case latency}
%
%In this section, We illustrate performance benefit of our scheduling method based on the worst case latency to short deadline HWA against
%by comparing other two methods.
%First method (SQUASH-TDistSh) always prioritizes the short deadline HWA against all CPUs and long deadline HWAs.
%%If the short deadline HWA
%%is not memory intensive, interference from the short deadline HWA to other requestors will be small.
%Second method (SQUASH-TDist0.8) is SQUASH-TDist with {\it EmergentThreshold} of 0.8.
%%is scheduling the short deadline HWAs using the dynamic priority~\cite{schedulingCPUGPU},
%The last one (SQUASH-Sh) employes scheduling based on the worst case latency to short deadline HWA. In the all methods, long
%deadline HWAs are scheduled with \emph{Dist-Prio}.
%
%Figure\ref{plot:emerge_performance} shows the system performance with the three scheduling algorithms for Config-A.
%We execute 10 workloads for each memory intensity of CPU workloads. Over the all workloads, the deadline met ratio of HES-HWA is 100\%.
%We have two conlusions. First, SQUASH-Sh achieves performance improvement by 3\% at maximum over the other algorithms due to delaying
%giving high priority to the HWA. Second, SQUASH-TDistSh and SQUASH-TDist0.8 shows almost the same performance. This is because, once HES-HWA becomes
%high priority, it utilizes most of requests and finishes much earlier than deadline prior to the other requestors.
%We conclude that scheduling method with the worst case latency is effective to improve system performance.
%
%\begin{figure}[ht!]
%  \centering
%  \begin{minipage}{0.32\textwidth}
%    \centering
%    \includegraphics[scale=0.22, angle=270]{plots/emerge_results_ws}
%  \end{minipage}
%  \caption{System performance with QoS-aware scheduling algorithms}
%  \label{plot:emerge_performance}
%\end{figure}

\subsection{Sensitivity Analysis}
%\subsubsection{Threshold for TCM}
%
%Figure~\ref{plot:threshold_results} shows the system performance, fairness and deadline met ratio of TCM-DynD, SQUASH and SQUASH-Prob
%with different threshold that is used to classify memory intensive applications and memory non-intensive applications, across combinations of 5 CPU workloads
%and 24 HWA configurations shown in Table\ref{tab:hwa_comb_config}. All performance and fairness are normalized
%with TCM-DynD-0.2. The result indicates that bigger threshold value generally improves system performance and degrade fairness. Bigger threshold allows that more applications
%are executed prior to non-urgent HWAs, but memory intensive applications have to compete for limited bandwidth. Moreover, with SQUASH and SQUASH-Prob, non-urgent HWA is higher priority
%than memory-intensive applications and bandwidth for memory intensive applications is quite limited. Therefore, higher threshold leads to higher unfairness.
%
%\begin{figure*}[ht!]
%  \centering
%  \begin{minipage}{0.24\textwidth}
%    \centering
%    \includegraphics[scale=0.16, angle=270]{plots/threshold_ws}
%  \end{minipage}
%  \begin{minipage}{0.24\textwidth}
%    \centering
%    \includegraphics[scale=0.16, angle=270]{plots/threshold_hs}
%  \end{minipage}
%  \begin{minipage}{0.24\textwidth}
%    \centering
%    \includegraphics[scale=0.16, angle=270]{plots/threshold_ms}
%  \end{minipage}
%  \begin{minipage}{0.24\textwidth}
%    \centering
%    \includegraphics[scale=0.16, angle=270]{plots/threshold_met}
%  \end{minipage}
%  \caption{Sensitivity to threshold for TCM}
%  \label{plot:threshold_results}
%\end{figure*}

\subsubsection{Number of Channels}

Figure~\ref{plot:ch_num_results} shows the system performance, fairness and deadline met ratio of FRFCFS-Dyn0.3, SQUASH and SQUASH-Prob with different number of channels across 25 CPU workloads with
HWA Config-A when all other parameters are the same as baseline. We make two observations from this result.
First, the benefit for system performance and deadline met ratio of SQUASH and SQUASH-Prob is decreased as the number of channels is increased. Because the large number of channels reduces contention of memory,
CPUs can utilize a large amount of bandwidth even when HWAs have high priority. For the same reason, the difference of fairness is decreased.
Second, SQUASH-Prob shows greater performance than that of SQUASH when ther number of channel is 4 or 8. This is because, non-urgent HWA can consume enough bandwidth to have good progress even if
priority of the HWA is lower than memory-intensive applications. In this case, SQUASH degrades the performance of memory-intensive applications. SQUASH-Prob prevent this degradation with
control probabilities.

\begin{figure}[ht!]
  \flushleft
  \begin{minipage}{0.23\textwidth}
    \flushleft
    \includegraphics[scale=0.16, angle=270]{plots/ch_num_ws}
  \end{minipage}
%  \begin{minipage}{0.24\textwidth}
%    \centering
%    \includegraphics[scale=0.16, angle=270]{plots/ch_num_hs}
%  \end{minipage}
  \begin{minipage}{0.23\textwidth}
    \flushleft
    \includegraphics[scale=0.16, angle=270]{plots/ch_num_ms}
  \end{minipage}
  \caption{Performance sensitivity to the number of channels}
  \label{plot:ch_num_results}
\end{figure}

\begin{figure}[ht!]
  \flushleft
  \begin{minipage}{0.23\textwidth}
    \flushleft
    \includegraphics[scale=0.16, angle=270]{plots/ch_num_methes}
  \end{minipage}
  \begin{minipage}{0.23\textwidth}
    \flushleft
    \includegraphics[scale=0.16, angle=270]{plots/ch_num_metmat}
  \end{minipage}
  \caption{Deadline met ratio sensitivity to the number of channels}
  \label{plot:channel_num_ratio}
\end{figure}

\subsubsection{Number of Cores}

Figure~\ref{plot:core_num_results} shows the system performance, fairness and deadline met ratio of FRFCFS-Dyn0.3, SQUASH and SQUASH-Prob
with different number of cores and HWAs across 25 CPU workloads when all other parameters are the same as baseline. The number of HWAs is 4 or 8.
When 4 HWAs, the configuration of HWAs is Config-A. The configuration of 8HWAs are IMG-HWA x2, MAT-HWA(10) x1, MAT-HWA(20) x1,
HES-HWA(32) x1, HES-HWA(128) x1, RSZ-HWA x1, DET-HEA x1. we have four conclustion from this result.
First, the weighted speedup and unfairness increase with increasing number of requestors. Second, The system performance benefits
of SQUASH incrase with increasing requestor count, because increasing requestor count lead to high memory contention and HWAs interfere
CPU cores. SQUASH mitigates interference with CPU applications from HWAs.

Third, when the number of HWAs is increased, unfairness of SQUASH become greater. This is because, many non-urgent HWAs most of bandwidth and
memory intensive applications have to compete remaining small amount of bandwidth. However, SQUASH-Prob can mitigate increasing of unfairness.

Finally, SQUASH and SQUASH-Prob keeps high deadline met ratio for every case.

\begin{figure}[ht!]
  \flushleft
  \begin{minipage}{0.23\textwidth}
    \flushleft
    \includegraphics[scale=0.16, angle=270]{plots/core_num_ws}
  \end{minipage}
%  \begin{minipage}{0.24\textwidth}
%    \centering
%    \includegraphics[scale=0.16, angle=270]{plots/core_num_hs}
%  \end{minipage}
  \begin{minipage}{0.23\textwidth}
    \flushleft
    \includegraphics[scale=0.16, angle=270]{plots/core_num_ms}
  \end{minipage}
  \caption{Performance sensitivity to the number of cores}
  \label{plot:core_num_results}
\end{figure}

\begin{figure}[ht!]
  \flushleft
  \begin{minipage}{0.23\textwidth}
    \flushleft
    \includegraphics[scale=0.16, angle=270]{plots/core_num_methes}
  \end{minipage}
  \begin{minipage}{0.23\textwidth}
    \flushleft
    \includegraphics[scale=0.16, angle=270]{plots/core_num_metmat}
  \end{minipage}
  \caption{Deadline met ratio sensitivity to the number of cores}
  \label{plot:core_num_ratio}
\end{figure}

\subsubsection{Scheduling and Unit}

We sweeped different values of scheduling unit and switching unit for SQUASH and SQUASH-Prob. We evaluate 500, 1000, 2000 and 5000 cycles for scheduling unit,
and 500, 1000, 2000 cycles for switching unit which is less than scheduling unit. We have three trends from the result.
First, when scheduling unit is 5000 cycles, MAT-HWA fails keeping the deadline met ratio 100\%, because it cannot absorb sudden bandwidth increase from other requestors.
Second, As the scheduling unit increases, the system performance is decreased. This is because, once HWA is deemed as urgent, HWA occupy memory bandwidth and interfere all CPUs for longer
time with bigger scheduling unit.

Third, when scheduling unit is fixed, smaller switching unit shows better fairness. Fine-grained probability control of SQUASH-Prob increases
the chance for memory-intensive CPU applications to get higher priority than non-urgent HWAs. Therefore, we have chosen 500 cycles for scheduling unit of SQUASH and
1000 and 500 cycles for scheduling unit and switching unit of SQUASH

%Figure~\ref{plot:schedulingunit_results} shows the system performance, fairness and deadline met ratio of SQUASH(SQ) and SQUASH-Prob(SQ-P)
%with different scheduling unit and switching unit. We execute 20 workloads for each unit and memory intensity of CPU workloads.
%On the legends, SQ-500 means that scheduling unit is 500 cycles and SQ-P-500/1000 means that scheduling unit is 500 cycle
%and switching unit is 1000 cycles. We have three observations for the results.
%First, coarser-grained scheduling cannot keep the deadline, because it
%Second, bigger scheduling unit introduces worse system performance.
%Even SQUASH-Prob, 5000 cycles of scheduling unit does not keep the dealine. This is because, probability control is gradual and it is not enough to absorb bandwidth fluctuation.

%\begin{figure}[ht!]
%  \flushleft
%  \begin{minipage}{0.23\textwidth}
%%    \centering
%    \flushleft
%    \includegraphics[scale=0.17, angle=270]{plots/scheduling_unit_performance}
%  \end{minipage}
%%  \begin{minipage}{0.24\textwidth}
%%    \centering
%%    \includegraphics[scale=0.16, angle=270]{plots/scheduling_unit_hs}
%%  \end{minipage}
%%  \begin{minipage}{0.24\textwidth}
%%    \centering
%%    \includegraphics[scale=0.16, angle=270]{plots/scheduling_unit_ms}
%%  \end{minipage}
%  \begin{minipage}{0.14\textwidth}
%    \flushleft
%    \includegraphics[scale=0.15, angle=270]{plots/scheduling_unit_avg_met}
%  \end{minipage}
%  \caption{Sensitivity to scheduling unit and switching unit}
%  \label{plot:schedulingunit_results}
%\end{figure}



==> sections/intro-lavanya.tex <==
\section{Introduction}

Today's mobile SoCs are heterogeneous architectures that integrate
hardware accelerators (HWA) and CPUs. Special purpose hardware
accelerators are widely used in SoCs, along with general purpose
CPU cores, because of their of ability to perform specific
operations in a fast and energy-efficient manner. For example, CPU
cores and Graphics Processing Units (GPUs) are often integrated in
smart phone SoCs. Hard-wired HWAs are implemented in a wide range
of SoCs\cite{visconti12}.  
% Citations are needed for current mobile SoCs besides Visconti2


%The HWAs are designed 
%so that target performance (e.g., frame rate) is satisfied in the design phase. However, HWAs share the memory subsytem with CPUs and HWAs cannot
%satisfy target performance due to interference form CPUs. Therefore, it is important and challenging to achieve
%high system performance while keeping HWAs' performance.


In several such SoCs, HWAs share the main memory with CPU cores. The main
memory is a heavily contended resource between multiple agents and
a critical bottleneck in systems. This becomes even more of a
problem since HWAs need to meet deadlines. Therefore, it is
important to manage the main memory such that HWAs meet deadlines
while still achieving high CPU performance.  

Several previous works have explored application-aware memory
request scheduling\cite{stfm,fair-queueing-memory,parbs,atlas,tcm},
reordering requests from different CPU cores to achieve high
performance and fairness. There have been few previous works that
have tackled the problem of main memory management in
heterogeneous systems with CPUs and hardware accelerators, with
the goal of meeting HWAs deadlines, while achieving good CPU
performance. In order to satisfy both CPUs' high performance and
HWAs' service quality (e.g., frame rate), memory controller needs
to be aware of their different requirements and access
characteristics. One relevant previous
work~\cite{schedulingCPUGPU} has tackled the problem of memory
management in CPU-GPU systems, striving to meet a target frame
rate for the GPU, while ensuring high CPU performance. The basic
idea of this work is to dynamically adjust CPU and GPU memory
access priorities based on periodically monitoring whether or not
the GPU is on track to meet the target frame rate. The scheduler
is aware of the different memory access requirements of CPU cores and HWAs. 
The paper makes the observation that CPU cores are more latency-sensitive than GPUs because GPUs can
hide their memory access latency with massive
multithreaded-execution. Therefore, GPU cores are given lower
priority by default, to minimize interference to latency-sensitive
CPU requests. However, in order to guarantee a target frame rate
to the GPU, the scheduler raises the GPU's priority when the GPU
is not making enough progress towards meeting its target frame
rate.

While such a scheme could potentially be adapted to meet the
deadline requirements of HWAs, we observe that such an approach
suffers from two fundamental shortcomings. First, when HWAs are
given high priority (based on monitoring their progress), they
cause significant interference to all CPU cores, degrading overall
system performance. Second, some HWAs have frequent deadlines
(short periods between deadlines). In such cases, deadlines are
missed when priorities are adjusted by tracking progress at a
coarse time granularity.   


\textbf{Our goal}, in this work, is to design a memory scheduler
that takes into account the differences in memory access
characteristics and demands of different CPU cores and HWAs, to
achieve high performance for CPUs while meeting HWAs' deadlines.
Towards this end, we propose a new QoS-aware memory scheduler for
heterogeneous systems, SQUASH, based on two key observations/ideas.

First, HWAs are prioritized over memory-intensive CPU
cores, even when HWAs are on track to meet their deadlines. We
observe, as also did several previous works~\cite{atlas,tcm}, that
memory-intensive CPU cores spend a significant fraction of their
execution time waiting for main memory and hence, delaying their
requests for a short time does not impact their performance
significantly. In fact, prioritizing HWAs over such
memory-intensive CPU cores reduces the amount of time HWAs are
not on track to meet their deadlines, thereby reducing the amount
of time they are prioritized over non-memory-intensive CPU cores
that are latency-sensitive. Second, short deadline HWAs are given
high priority, as their deadlines approach, based on worst-case
access latency calculations. This enables them to meet their
deadlines more effectively than a coarse-grained progress
measurement based scheme, while also reducing interference with
CPU cores.


This paper makes the following main contributions.

\begin{itemize}
\item{We present characteristics of HWAs and describe the issues with current
memory scheduling policies in terms of meeting HWAs deadlines, while improving
CPU performance.}
\item{We propose SQUASH, a new QoS-aware memory scheduling that improves the CPU
erformance while meeting HWAs deadlines. }
\item{We evaluate our proposed QoS memory scheduling against two existing priority
schemes and three memory scheduling policies. Our scheduling improved the system
performance by ??\% while meeting HWAs' deadlines.}
\end{itemize}



==> sections/mechanism-lavanya.tex <==
\section{Mechanism}

In this section, we describe the details of SQUASH, our proposed
memory scheduling mechanism to manage memory bandwidth between CPU
cores and HWAs. First, we will describe a scheduling policy to
prioritize between HWAs with long deadline periods and CPU cores,
with the goal of improving overall system performance while
enabling the long-deadline-period HWAs to meet their deadlines.
Next, we will describe how SQUASH enables HWAs with short deadline
periods to meet their deadlines. We will then describe a
modification to our original scheduling policy to
probabilistically change priorities between long-deadline-period
HWAs and CPU cores and enable higher fairness among CPU cores.

\textbf{Overview:} SQUASH categorizes HWAs as long-deadline-period and
short-deadline-period statically. A different scheduling policy is
employed for each of these two caterogies, since they have
different kinds of bandwidth demand. For the long-deadline-period
accelerators, SQUASH monitors their progress periodically and
appropriately prioritizes them, enabling them to get sufficient and
consistent bandwidth to meet their deadlines. For the
short-deadline-period accelerators, SQUASH gives them a short
burst of highest priority close to each deadline, based on
worst-case access latency calculations.

\subsection{Long-Deadline-Period HWAs vs. CPU Applications}
\label{sec:longdeadline}


SQUASH monitors each HWA's {\it CurrentProgress} and {\it
ExpectedProgress}, as defined in Equation~\ref{eq:HWAProgress},
every {\it SchedulingUnit}. At the end of a {\it SchedulingUnit},
{\it CurrentProgress} and {\it ExpectedProgress} are compared.
When {\it CurrentProgress} is less than or equal to {\it
ExpectedProgress}, the HWA is classified as urgent. Otherwise, it
is classified as non-urgent. Furthermore, apart from the progress
based urgency computation, after an {\it EmergentThreshold}
(90\% of the deadline period in our experiments), a
long-deadline-period HWA is classified as urgent.

CPU applications' memory-intensity is monitored during each {\it
SchedulingUnit}.  At the end of a {\it SchedulingUnit},
applications are classified as memory-non-intensive or
memory-intensive based on their calculated memory-intensity using
the classification mechanism employed in TCM~\cite{tcm}. Note that
other mechanisms can also be employed to perform this
classification.

Based on these HWA and CPU application classifications, requests
are scheduled at the memory controller in the following priority
order:

\begin{enumerate}
\item{Urgent HWAs}
\item{Memory-non-intensive CPU applications}
\item{Non-urgent HWAs}
\item{Memory-intensive CPU applications}
\end{enumerate}

Based on our first observation in Section~\ref{sec:obs1},
HWAs' requests are prioritized over memory-intensity CPU
applications' requests, when the HWAs are not deemed urgent,
since memory-intensive applications are not as latency-sensitive. 

\subsection{Providing QoS to HWAs with Short Deadline Periods}
\label{sec:shortdeadline}

While HWAs with long-deadline-periods can often get a consistent
share of memory bandwidth and meet their deadlines, through a
scheme that monitors progress and appropriately assigns
priorities, HWAs with short deadline periods do not get a
consistent share of memory bandwidth with such a scheme (as we
described in our second observation in Section~\ref{sec:obs2}).
In order to enable HWAs with short deadline periods to meet their
deadlines, we propose to give them a short burst of high priority
close to a deadline, based on worst case latency calculations.

\textbf{Calculating worst case access latency:} In the worst case,
all requests from a short-deadline-period HWA would access the
same row on a bank. In this case, all such requests are serialized
and each request takes tRC - the minimum time between two DRAM row
ACTIVATE operations.\footnote{Accesses to two DRAM rows on the
same bank have to be spaced apart by tRC.} Therefore, in order to
serve the requests of a short-deadline-period HWA before its
deadline, it needs to be deemed urgent and given the highest
priority over all other agents for $tRC*TheNumberOfRequests$ for
each period. We call this high priority period the
$WC\mathchar`-MAL$ (Worst-Case Maximum Access Latency period). For
example, when a HWA outputs 16 requests every 2000 ns period and
tRC is 50 ns, the HWA is deemed urgent and given the highest
priority for 800 ns + $\alpha$ during each period, where $\alpha$
is the waiting time for an ongoing request to finish. Furthermore,
finishing a HWA's requests much earlier than the deadline is
wasteful, since it does not improve the HWA's performance any
further. Hence, this highest priority period can be at the end of
the HWA's deadline period. For instance, in the previous example,
the HWA is given highest priority (1200-$\alpha$) after a deadline
period starts. 

\textbf{Handling multiple short-deadline-period HWAs:}
While the scheme discussed above would work when there is a single
short-deadline-period HWA, when multiple short-deadline-period
HWAs are present, it could cause overlap in high priority cycles
between them resulting in deadline misses. We propose to address
this concern using the following mechanism:

\begin{enumerate}
\item
The urgent period of each HWA x for a deadline period, is calculated first as 
$WC\mathchar`-MAL(x) = tRC*TheNumberOfRequests(x)$
\item
The urgent period of each HWA x, is extended by a scaled
version of the $WC\mathchar`-MAL$, of all HWAs that have higher
priority than HWA x, in order to ensure that each HWA is given
highest priority for enough cycles. Specifically, 

$WC\mathchar`-MAL(x) = \Sigma_i (WC\mathchar`-MAL(x)/Period(i)) *
WC\mathchar`-MAL(i) + WC\mathchar`-MAL(x)$, 

for all HWAs i with that have shorter deadline periods than HWA x.
\item
Among the urgent short-deadline-period HWAs, the HWAs with shorter
deadline periods are given higher priority.
%\nonumber
\end{enumerate} 

Such a mechanism provisions for enough urgency for each HWA, even
if its urgent period overlaps with other HWAs' urgent periods.

\subsection{Overall Scheduling Policy}
Combining the mechanisms described in
Sections~\ref{sec:longdeadline} and~\ref{sec:shortdeadline},
SQUASH schedules requests in the following order:

\begin{enumerate}
\item
\textbf{Urgent HWAs in the short deadline period group:} Higher
priority to shorter deadline HWAs
\item
\textbf{Urgent HWAs in the long deadline period group:} Higher
priority to earlier deadline HWAs
\item
\textbf{Memory-non-intensive CPU applications:} Higher priority to
lower memory-intensity applications
\item
\textbf{Non-urgent HWAs in the long deadline period group:} Higher
priority to earlier deadline HWAs
\item
\textbf{Memory-intensive CPU applications:} Randomly shuffled
priorities like TCM~\cite{tcm}
\item
\textbf{Non-urgent HWAs in the short deadline period group:}
Higher priority to shorter deadline HWAs
\end{enumerate}


%Lavanya: For now, I am not sure what's the best way to write this. One
%possibility is to explain the intra-group prioritization in the
%itemized list itself. The other possibility is to move it below,
%like Hiroyuki originally had. We can decide later, depending on
%what you all think.

%Between two HWAs having the same priority, rate monotonic
%scheduling that priorizies the HWA having shorter period is used
%for the short deadline group and early deadline first scheduling
%that prioritizes the HWA whose deadline is more closed is used for
%the long deadline group. Among CPUs in the same group, TCM is used
%to scheduling.

While this policy is effective in achieving close to 100\%
deadline meet rate while improving overall system performance in
most cases, memory-intensive applications experience unfair application
slowdowns, since they are ranked lower than all groups, except
non-urgent short-deadline-group HWAs. We propose a modification
to the SQUASH policy to enable higher fairness for
memory-intensive applications.

\subsection{Switching Long-Deadline-Period HWA Priorities Probabilistically}

In order to address unfair slowdowns of memory-intensive
applications, we propose a mechanism, SQUASH-Prob, to
probabilistically prioritize memory-intensive applications over
non-urgent HWAs and memory-non-intensive applications. 

The SQUASH-Prob mechanism switches probabilities between the
non-urgent long-deadline HWAs and memory-intensive applications.
Each long-deadline-period HWA has a probability value $Pb$ that is
controlled based on request progress. We will first describe how
requests are scheduled based on $Pb$ and then describe how $Pb$ is
controlled.

\textbf{Scheduling using $Pb$.}

With a probability $Pb$,\\
Memory-non-intensive applications $>$ Memory-intensive applications $>$
Long-deadline-period HWA\\

With a probability $(1-Pb)$,\\
Memory-non-intensive applications $>$ Long-deadline-period HWA $>$ Memory-intensive
applications\\

The long-deadline-period HWA is prioritized over memory-intensive
applications with a probability $Pb$, enabling higher fairness for
memory-intensive applications.

\textbf{Controlling $Pb$. }
At the beginning of execution, $Pb = 0\%$ (which would result in
the same scheduling order as the basline SQUASH policy).

Every {\it SwitchingUnit}, $Pb$ is increased or decreased
depending on whether the HWA is making sufficient progress, as
follows:

If {\it ExpectedProgress} > {\it CurrentProgress} $Pb$ is
incremented by $Pb_{inc}$ (1\% in our experiments).
If {\it CurrentProgress} > {\it ExpectedProgress} $Pb$ is
decremented by $Pb_{dec}$ (5\% in our experiments).

The decrement is larger than the increment since we want to reduce
priority to memory-non-intensive applications and increase the
HWA's bandwidth allocation rapidly when it is not making
sufficient progress.


%Lavanya: I skipped the part below in the explanation in the interest
%of reducing the complexity of the explanation. We can probably
%add a couple of sentences on it later (maybe even in the
%evaluation section)


%\subsection{Additional Scheduling Detail}
%The scheduling described in \ref{sec:SummaryOfScheduling} will not work well when all CPUs demands quite low bandwidth. 
%In this case a HWA can consume greater bandwidth than the demand when all CPUs are prior to the HWA. If the dynamic priority scheme is applied to the system, 
%the amount of time HWA has high priority is quite small. Therefore, the benefit for system performance of the SQUASH is limited. TCM compares memory intensity of CPU applications relatively and
%categorize some applications into memory intensive CPU applications in such situation. Consequently, SQUASH still delayes memory intensive applications and will degrade sytem perfomance.
%
%To prevent this problem, we apply our application-aware dynamic priority only when a HWA does not utilize enough bandwidth in low priority. 
%At the beginning of each period, we do not prioritize a HWA with low priority in long deadline group against CPUs in group-B. 
%The HWA have the same priority as HWAs with low priority in short deadline group. After detecting the HWA's priority transition from low to high, we prioritize
%the HWA with low priority against CPUs in group-B because it means HWA was not able to consume enough bandwidth in low priority. 



==> sections/motivation-lavanya.tex <==
\section{Motivation}

A similar policy, as the one proposed by Jeong et
al., in~\cite{schedulingCPUGPU} for CPU-GPU systems can be
applied to manage memory bandwidth between CPU cores and HWAs,
since HWAs have several characteristics that are similar to GPUs.
Similar to GPUs' frame rate requirements, HWAs need to meet
deadlines. Furthermore, like GPUs, HWAs also have higher memory
latency tolerance, because of the presence of scratch pad memory
such as line buffers and double buffers.

{\it CurrentProgress} for HWAs can be defined in terms of the
fraction of the total number of memory requests that have been
completed. For hard-wired HWAs, it is possible to precisely know
the number of memory requests that need to be served during each
period. {\it ExpectedProgress} for HWAs can be defined in terms
of the fraction of time elapsed during a deadline. 


\begin{eqnarray*}
CurrentProgress = \frac{\#\ of\ finished\ memory\ requests / period}{\#\ of\ total\ memory\ requests / period}\\
%\label{eq:Progress}
%\end{equation}
%\begin{equation}
ExpectedProgress = \frac{Time\ elapsed\ in\ the\ current\ period}{Total\ length\ of\ current\ period}
%\label{eq:ExpectedProgress}
\end{eqnarray*}

Furthermore, in order to better meet deadlines, the mechanism
in~\cite{schedulingCPUGPU} can be adapted to make the HWA enter a
state of urgency and give it highest priority, anytime when {\it
CurrentProgress} is equal to or lower than {\it ExpectedProgress}.

We examine the effectiveness of such a scheduling policy in a
system with a HWA and two CPU cores. Figure \ref{fig:singlemaster}
depicts the requests generated and the execution timeline when
each agent (HWA or CPU core) executes by itself. CPU-A has low
memory-intensity and generates very few memory requests. CPU-B has
high memory-intensity and generates many more memory requests than
CPU-A does. The HWA has double buffers and generates 8 prefetch
requests for the data to be processed in the next period. For ease
of understanding, we assume all these requests are destined to the
same bank and each memory request takes T cycles (no distinction
between row hits and misses). The period of the HWA is 16T. Every
4T time units, {\it CurrentProgress} and {\it ExpectedProgress}
are compared and the HWA's state of urgency and priority are
recomputed.

\begin{figure}
  \centering
  \includegraphics[scale=0.45, angle=0]{figs/fig_timing_alone}
  \caption{Memory service timeline example when each master is executed alone}
  \label{fig:singlemaster}
\end{figure}

Figure~\ref{fig:schedulingexample-dynamic} illustrates the
scheduling order of requests from the HWA and the two CPU cores,
when the dynamic priority mechanism~\cite{schedulingCPUGPU} is
employed. At the beginning of the deadline period, since both {\it
CurrentProgress} and {\it ExpectedProgress} are zero and equal,
the HWA is deemed as urgent and is given higher priority than the
CPU cores. Hence, during the first 4T cycles, only the HWAs
requests are served. After 4T cycles, {\it CurrentProgress} is 0.5
and {\it ExpectedProgress} is 0.25. Hence, the HWA is deemed as
not urgent and is given lower priority than the CPU cores.
Requests from both CPU cores are served during cycles 4T to 8T.
After 8T cycles, since both {\it CurrentProgress} and {\it
ExpectedProgress} are 0.50, the HWA is deemed urgent and given
higher priority than the cores. Hence, during cycles 8T to 12T,
the HWAs remaining four requests are completed, enabling the
completion of the CPU cores' remaining requests during cycles 12T
to 16T.

%Please split this figure into two subfigures. That would make it
%easier to refer to the two parts of the figure.

\begin{figure}
  \centering
  \includegraphics[scale=0.45, angle=0]{figs/fig_timing}
  \caption{Memory service timeline example}
  \label{fig:schedulingexample}
\end{figure}

While such a scheduling policy could potentially achieve high overall
system performance while also meeting the HWA's deadlines, we observe
that such a policy suffers from two major shortcomings.

First, the HWA causes significant interference to all CPU cores,
when it is deemed urgent and prioritized over all CPU cores.
Second, such a coarse grained progress based scheduling approach
could cause deadline misses for HWAs with short periods (frequent
deadlines). We will describe these two shortcomings and our
proposed solution directions in more detail in the next sections.

\subsection{Interference to All CPU Cores}

In the dynamic priority scheme discussed above, when a HWA is
deemed urgent, it is given higher priority over all CPU cores and
interferes with all CPU cores. For instance, in Figure
\ref{fig:schedulingexample-dynamic}, during cycles 8T to 12T, the HWA
stalls both CPU-A and CPU-B. Furthermore, the higher the memory
intensity of the HWAs, the more memory bandwidth they need to make
sufficient progress and meet their deadlines, causing significant
interference to the CPU cores. For example, when a
memory-intensive HWA that demands 8.32 GB/s of memory bandwidth
and generates streaming memory accesses to data in the same row
(on the same channel), when it shares a 2-channel DRAM memory
system with a peak bandwidth of 21.3 GB/s with eight CPU cores and
three other HWAs, the memory-intensive HWA is deemed urgent and
given highest priority 70\% of the execution time. When HWAs reach
a state of urgency and are given highest priority for such long
periods of time, CPU cores' performance degrades significantly. We
propose to tackle this shortcoming based on our first
observation.

\textbf{Observation 1:} Memory-intensive applications do not
experience significant performance degradation when they are
prioritized lower than HWAs.

Previous work~\cite{atlas,tcm} has observed that applications with
low memory-intensity are more sensitive to memory latency, since
these applications generate few memory requests and quick service
of these few requests enables the application to make good forward
progress. On the other hand, applications with high
memory-intensity often have a large number of requests outstanding
at the main memory and spend a significant fraction of their
execution time stalling on main memory. Therefore, delaying high
memory-intensity applications' requests does not impact their
performance significantly. Hence, we propose to prioritize HWAs'
memory requests over those of high memory-intensity applications
even when HWAs are making sufficient progress and are not deemed
urgent. Such a prioritization scheme would reduce the number of
cycles when the HWAs are deemed urgent and prioritized over
latency-sensitive low memory-intensity applications, thereby
reducing the interference caused to such applications.

Figure~\ref{fig:schedulingexample-squash} illustrates the benefits
of such an application-aware dynamic priority scheme for the same
set of requests as shown in
Figure~\ref{fig:schedulingexample-squash}. The request schedule
remains the same from times 0 to 4T. At time 4T, the {\it
CurrentProgress} is 0.5 and {\it ExpectedProgress} is 0.25. Since
the {\it CurrentProgress} is lower than {\it ExpectedProgress},
the HWA is not deemed urgent and CPU-A's request is prioritized
over the HWA's requests. However, the HWA is \emph{still}
prioritized over CPU-B that has high memory-intensity. As a
result, at time 8T, {\it CurrentProgress} is 0.875 and is greater
than {\it ExpectedProgress} and the HWA is still deemed not
urgent, unlike in the baseline case (in
Figure~\ref{schedulingexample-dynamic}). Hence, the
latency-sensitive CPU-A's requests are served earlier, enabling
faster progress for CPU-A, as can be seen from
Figure~\ref{fig:schedulingexample-squash} and higher overall system
performance

\subsection{Deadline Misses for Short Deadline HWAs}

Monitoring progress periodically and appropriately adjusting
urgency and priorities is an effective mechanism to ensure
consistent bandwidth to HWAs that have fairly long periods
(infrequent deadlines). However, such a scheme is not effective
for HWAs with short periods (frequent deadlines) since it is
difficult to ensure that these HWAs are deemed urgent and receive
enough priority for sufficiently long periods of time such that
they meet their deadlines. Specifically, they are susceptible to
interference from other HWAs and CPU cores and their available
memory bandwidth fluctuates. Figure~\ref{fig:hwa-remaining} shows
how many cycles ahead of a deadline are all memory requests
generated during that deadline period completed for two HWAs,
HWA-A and HWA-B. HWA-A has a long deadline period (63041 Cycles)
and demands significant memory bandwidth (8.32 GB/s). HWA-B has a
short deadline period (5447 Cycles) and demands much lower memory
bandwidth (478 MB/s). HWA-A's memory requests are completed ~1500
cycles before the deadline and there is not much variability in
this behavior across time. On the other hand, HWA-B's (the short
deadline period accelerator) deadline is highly variable to the
point of causing a few deadline misses, demonstrating that HWAs
with short deadline periods are susceptible to bandwidth
fluctuations caused by other other HWAs and CPU cores. We propose
to tackle this shortcoming using our second observation.

\begin{figure}
  \centering
  \includegraphics[scale=0.35, angle=0]{figs/fig_remaining}
  \caption{Remaining cycles for a period when all requests are finished}
  \label{fig:hwa-remaining}
\end{figure}

\textbf{Observation 2:} {\it Short deadline HWAs can be enabled to 
meet their deadlines by giving them a short burst of highest
priority very close to the deadline.}

In order to meet its deadline, a short deadline HWA requires
guaranteed priority for enough time such that all its requests can
be completed by the deadline. We propose to achieve this by
estimating the $WorstCaseLatency$ for a memory access and giving a
short deadline HWA highest priority for
$NumberOfRequests*WorstCaseLatency$ cycles close to the deadline.
This burst of highest priority does cause interference to all CPU
cores. To mitigate this interference, we propose to delay this
high priority burst very close to the deadline, since finishing
requests earlier than the deadline does not improve the HWA's
performance.

Based on these two observations, we propose a new QoS-aware memory scheduler
design, SQUASH, that aims to meet HWAs' deadlines while improving
overall system performance. We will describe the details of the
memory scheduling mechanism in the next section.



==> sections/qualitative-comparison.tex <==
\subsection{Qualitative Comparison with Previous Schedulers}

We compare SQUASH qualitatively compare SQUASH with the other QoS-aware schedulers. 
A Predictable SDRAM Memory Controller(Predator)~\cite{predator} guarantees 
a minimum bandwdith and a maximum latency for each requestors. Predator is based on the
two technuques. First, Predator groups one read or write burst to all banks and schedules
each group of requests together in order to improve bandwidth utilization. Second, 
Credit-Controlled Static Priority (CCSP) arbiter~\cite{ccsp} is used to schedule requests at the memory
controller using a rate-based regulation scheme and a static priority scheduler.
Unlike SQUASH, predator does not consider memory characteristics of different kinds of masters.
A designer has to explore the best configurations for CPU applications manually. 
Moreover, grouping requests to all banks degrades flexiblity, because requests to the same bank
are not scheduled consecutively even if they hit row-buffer. Therefore, it leads to low utiliztion.

Memguard~\cite{memguard} divides memory bandwidth into two components - a guaranteed component and
a best-effort component. A certain guaranteed component of
bandwidth is ensured for each core. After each core consumes its
guaranteed bandwidth, the remaining bandwidth is used to achieve
good performance, in a best-effort manner.
As with Predator, Memguard does not consider memory characteristics of masters.
Both Memguard and SQUASH guarantees bandwidth based on the worst case latency, but Memguard 
can not guarantee more bandwidth than that based on the worst case latency. The HWA that require
a large amount of bandwidth executes in only a best-effort manner and will sometimes fail the deadline.
On the other hand, SQUASH can guarantee consistent bandwidth by adjusting priority.

In contrast to these QoS-aware schedulers, SQUASH improves CPU applications' performance by considering
memory characteristics of CPUs and HWAs while keeping HWAs' deadline with two different priority scheme
based on the deadline.



==> sections/sq_component.tex <==

\begin{table}[h!]
\scriptsize
\centering
\begin{tabular}{|l|l|}
  \hline
  Configuration & Description \\
  \hline
  \hline
  SQ-D & distributed priority on top of TCM for CPU applications\\
  \hline
  SQ-D+L & SQ-D along with application-aware prioritization between \ldphwas and memory-intensive CPU applications \\
  \hline
  SQ-D+L+S & SQ-D+L along with worst-case latency based prioritization for \sdphwas \\
  \hline
  SQ-D+L+S+P & Complete SQUASH mechanism, SQ-D+L+S along with probabilistic prioritization between \ldphwas and memory-intensive CPU applications \\
  \hline
  \end{tabular}
  \vspace{-2mm}
  \caption{SQUASH Configuration}
  \label{tab:sq_component}
\end{table}

